FPDetect: Efficient Reasoning About Stencil Programs Using Selective Direct Evaluation

We present FPDetect, a low overhead approach for detecting logical errors and soft errors affecting stencil computations without generating false positives. We develop an offline analysis that tightly estimates the number of floating-point bits preserved across stencil applications. This estimate rigorously bounds the values expected in the data space of the computation. Violations of this bound can be attributed with certainty to errors. FPDetect helps synthesize error detectors customized for user-specified levels of accuracy and coverage. FPDetect also enables overhead reduction techniques based on deploying these detectors coarsely in space and time. Experimental evaluations demonstrate the practicality of our approach.

==> error-analysis.tex <==

\begin{comment}
In the interest of space, we present a high
level version in the main
body\footnote{Our supplementary material
  has more details.}.
\end{comment}

Our error analysis methods build upon
the works of~\cite{higham,boldo} but are
appled to much larger expressions.
%
Our goal is to define
detector precision$(dp_T)$ for the T-step lookahead detector.
%
A first order affine model is used to model floating point error.


\ggcmt{Shrink this para to half its size.}
A floating point number system, $\mathbb{F}$ , in radix, $\beta$, is a subset 
of the set of real numbers, and can be expressed as a 5 tuple $(\beta, s,m,e,p)$.
We use binary ($\beta=2$) double precision with $p=53$.
$s \in \{-1,1\}$ is the sign bit, $e$ is the exponent in the range $-1022 \leq e \leq 1023$,
and $m$ is the mantissa or the significand, and represents
the magnitude $s\cdot m \cdot 2^e$.
%
If $x \in \mathbb{R}$, then $x_f \in \mathbb{F}$ denotes an element in $\mathbb{F}$ closest to $x$ obtained
by applying the rounding operator $(\circ)$ to $x$. We use the bound consistent 
for all IEE754~\cite{ieee754} rounding modes.
%IEEE754 defines four rounding modes for elementary 
%floating point operations namely rounding towards positive infinity $(\circ_{+\infty})$, towards
%negative infinity $(\circ_{-\infty})$, towards zero $(\circ_0)$ and to the nearest $(\circ_\backsim)$.
%Every real number $x$ lying in the range of $\mathbb{F}$ can be approximated by an element  $x_f \in \mathbb{F}$
%with a relative error no larger than the {\em unit roundoff} $\boldsymbol{u} = \dfrac{1}{2}\beta^{1-p}$. 
%Here $\beta^{1-p}$ corresponds to the {\em unit of least precision(ulp)} for exponent value of 1.
%We use $\mu$ to denote ulp(1), such that $\mu = 2\boldsymbol{u}$.
%In our case $\boldsymbol{u} = 2^{-53}$, and hence $\mu = 2^{-52}$. 
%Hence, for all $\circ \in \{\circ_{+\infty},\circ_{-\infty},\circ_0, \circ_\backsim \}$, 
%we have the following result
Every real number $x$ lying in the range of $\mathbb{F}$ can be approximated by an element  $x_f \in \mathbb{F}$
with a relative error no larger than the {\em unit roundoff} $\boldsymbol{u} = 0.5\times\beta^{1-p}$. 
Here $\beta^{1-p}$ corresponds to the {\em unit of least precision(ulp)} for exponent value of 1.
We use $\mu$ to denote ulp(1), such that $\mu = 2\boldsymbol{u}$.
In our case $\boldsymbol{u} = 2^{-53}$, and hence $\mu = 2^{-52}$. 
Hence, for all rounding modes($\circ$), 
\( \circ(x) = x(1 + \delta),\quad |\delta| \leq \boldsymbol{u} = \mu/2.\)
Given two exactly represented floating point numbers $x_f$ and $y_f$,
arithmetic operators $\diamond \in \{ +,-,\times\}$ have the following guarantees across
any rounding modes:
\(
x_f \diamond_f y_f = (x_f \diamond y_f)(1 + \delta),\quad |\delta| \leq 2\boldsymbol{u} = \mu.\)

\noindent{\bf Affine Arithmetic:\/}
We use
{\em Affine Analysis(AA)}~\cite{stolfi} that partially adresses the 
loss of correlation. In an affine representation 
$\hat{x} = x_0 + \sum_{i=1}^n x_i \epsilon_i $, 
%
$x_0$ denotes the central value of the corresponding interval
and coefficients $x_i$ are finite floating
point numbers. The $\epsilon_i$ are {\em formal noise variables} which are unknown until concretized but assumed to lie in the interval [-1,+1].

% what all we must present minimally ?
% add and mult model with noise vars
% sigmal, gamma definitions
% stenci

%--\noindent{\bf Affine model for Floating Point operations:\/}
%Equation $\eqref{eq:rounding}$ shows the relation between a real number $x$ 
%and its rounded floating point representation $x_f$. 
We model the round-off error as a formal noise variable whose 
value lies in range [-1,1] and an asociated noise coefificent. 
The value that a noise variable may ultimately take determines the fraction
of the noise coefficient that actually contributes to the round-off error:
\( 	x_f = \circ(x) = x(1 + \delta) =
 x + (x\boldsymbol{u})\epsilon;\quad |\delta| \leq \boldsymbol{u};\quad \epsilon \in [-1,+1]. \)
 \ggcmt{Here it is {\bf{\em u}} while below it is
   {\bf$\mu$}. Why? }
   
\noindent{\bf Operators to retrieve noise variables and coefficients:\/}
Let {\em $\sigma$} be a
mapping from an error laden floating point  variable 
to its set of nosie variables.
Thus if $x_f$ is laden with $n$ noise variables,
then		$\sigma({x_f}) = \{\epsilon_i\}_{i=1}^n$.
%
Let {\em $\sigma^{(0)}$} be a special case of $\sigma$ to retrieve {\em freshly generated
  noise variables} during a floating point operation.
We utilize this notion for separation and propagation of error terms.
%
Also, let $\gamma$  be a mapping from a 2-tuple of
{\em (float variable, noise variable)} to its
corresponding noise coefficient. Thus,
\( \gamma(x_f, \epsilon_i) = 
x_i if \epsilon_i \in \sigma(x_f)\), and $0$ otherwise.
%
Now,
two error-laden floating point variables, $x_f$ and $y_f$ can be represented per our model 
as 
 \begin{equation}
 \label{eq:affine-float-representation}
 \begin{split}
 	x_f &= x + \sum_{\epsilon_i \in \sigma(\hat{x})} \gamma(\hat{x}, \epsilon_i)\epsilon_i \ ;\quad
 	y_f = y + \sum_{\epsilon_i \in \sigma(\hat{y})} \gamma(\hat{y}, \epsilon_i)\epsilon_i \\
 \end{split}
 \end{equation}

Let $\alpha$ and $\beta$ be two exactly represented scalar quantities. 
Every floating point operation,
 $\diamond_f \in \{\circ(+), \circ(-), \circ(\times) \}$ introduces a 
 {\em fresh noise variable}($\epsilon_{new}$) with 
 coefficients equal to the uncertainty of maximum round-off error introduced by that operation as
 in $\eqref{eq:opbound}$.
 We consider two operations specific to the stencil inner product:
 (1) scaling $x_f$ by an exactly represented scalar $\alpha$ shown in 
 $\eqref{eq:affine-float-mult}$, and
 (2) add or subtract two error-laden FP numbers $x_f$ and $y_f$ as shown in 
 $\eqref{eq:affine-float-add}$
 %
 \vspace*{-0.4em}
 \begin{equation}
 %\label{eq:affine-float-operations}
 \label{eq:affine-float-mult}
 \begin{split}
   \circ(\alpha{\!} \times{\!} x_f) &=\! \bigg (\alpha x\! +{\rs\rs\rs}\sum_{\epsilon_i \in \sigma(x_f)}{\rs\rs} \alpha \gamma(x_f,\epsilon_i)\epsilon_i
   							  \bigg )\! 
 							   +\! \boldsymbol{((\alpha x)\mu)}\epsilon_{new}\! +\! \{\mbox{he}\} 
 \end{split}
 \end{equation}
 
 \vspace*{-0.4em}
 \begin{equation}
 \label{eq:affine-float-add}
 \begin{split}
 	\circ(x_f{\!} +{\!} y_f) &= (x+y) +{\rs\rs\rs} \sum_{\epsilon_i \in \sigma(x_f)\cup\sigma(y_f) } {\rs\rs\rs}\{\gamma(x_f,\epsilon_i) + \gamma(y_f,\epsilon_i) \}\epsilon_i  
 			  \quad +\boldsymbol{((x+y)\mu)}\epsilon_{new} + \{\mbox{he}\}
 \end{split}
 \vspace*{-0.4em}
 \end{equation}

 The scaling in $\eqref{eq:affine-float-mult}$ and the 
 superposition of the coefficients in $\eqref{eq:affine-float-add}$ over the 
 union of the noise variables depicts the propagation of existing noise variables
 in addition to the generation of fresh noise variables.
 Tracking this distinction allows us to treat {\em error propagation}
 and {\em error gneration} separately
 as introduced by Darulova~\cite{Comp-for-reals}.
 \ggcmt{You said this is found in another place also?
   So maybe say ...
   separately~cite{cite1,darulova-as-second-cite}?}
 %
 We analyze the effect of each individual formal noise variable
 separately instead of over-approximating all error terms together as done in IA.
 

 Consider a real function $f$ and its floating point version $\tilde{f}$. 
 The real set of variables is denoted by 
 $\mathbf{x}$ while the rounded off variable set(with error laden terms) are denoted as
 $\mathbf{\tilde{x}}$. The total error can be written and decomposed in the form
 \begin{equation}
 \label{eq:darulova-separation}
 \begin{split}
 	|f(\mathbf{x}) - \tilde{f}(\mathbf{\tilde{x}})| &\leq \overbrace{|f(\mathbf{x}) - f(\mathbf{\tilde{x}})|}^\text{propagation of errors} + 
 											\overbrace{|f(\mathbf{\tilde{x}}) - \tilde{f}(\mathbf{\tilde{x}})|}^\text{Freshly generated errors}
 \end{split}
 \vspace*{-0.4em}
 \end{equation} \\ [-1em]

The first term represents the contribution of the initial error in the input
to the output. Each input variable associates with itself a propagation factor
by which error on the input gets propagated. This factor essentially depends 
on the the derivative of the function with respect to the 
input points. Let $K_i$ denote the propagation factor for variable $x_i$ and 
$\sigma_i$ denotes the set of noise variables existing at $x_i$ as part of
the incoming error. Then 
\vspace*{-0.2em}
 \begin{equation}
 \label{eq:slope-propagate}
 \begin{split}
   |f(\mathbf{x}) - f(\mathbf{\tilde{x}})| &\leq \sum_{i=1}^m K_i \bigg ( \sum_{\epsilon_i \in \sigma(x_i)} \gamma(x_i,\epsilon_i)\epsilon_i \bigg )\ ;\quad
   \mbox{where, } K_i = \underset{w_i \in\ \mathbf{\tilde{x}}}{sup} \bigg | \dfrac{\partial f}{\partial w_i}\bigg | \\
 \end{split}
 \vspace*{-1em}
 \end{equation}
 %
 Evaluating $K_i$ factors is easy to visualize once the computational graph is available as shown in ~\ref{fig:cfg}.

   As a simple ilustration, consider a single step iteration of a 1-d 3-point stencil with stencil coefficients
  $\{c_1, c_2, c_3 \}$ centered around $x_2$ to evaluate $x_2$ for the next time step, denoted here as S in Figure$~\ref{fig:cfg}$.
  Thus the computational graph evaluates $S=((c_1\times x_1)+(c_2\times x_2))+(c_3\times x_3)$. If $\epsilon^\prime$
  is a noise variable belonging to $\sigma(x_1)$ , then the error contribution's propagation at $S$ will be
  \begin{equation}
  \label{eq:chain-rule}
  \begin{split}
  	\gamma(\epsilon^\prime)\cdot K_{x_1} &=  \gamma(\epsilon^\prime)\cdot \bigg| \dfrac{dS}{dx_1}\bigg| 
  	                                     =  \gamma(\epsilon^\prime)\cdot \bigg| \dfrac{dS}{dS}\cdot
 										 	\dfrac{dS}{dq}\cdot
 											\dfrac{dq}{dz_1}\cdot
 											\dfrac{dz_1}{dx_1}\bigg| 
 										= \gamma(\epsilon_i)\cdot 1 \cdot 1 \cdot 1 \cdot c_1 
 										 = \gamma(\epsilon_i) \cdot c_1
  \end{split}
  \end{equation}
  Thus for all such $\epsilon^\prime \in \sigma(x_1)$, the $\gamma(x_i, \epsilon^\prime)$ gets propagated by $c_1$.
  Similarly for $x_2$ and $x_3$.


\begin{figure}
    \centering
    \begin{minipage}{0.45\textwidth}
\includegraphics[width=0.85\columnwidth]{figs/computationalGraph}\\
\caption{\label{fig:cfg}
Computational graph with highlighted derivatives for 1 step of a 1-d 3-point stencil
}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
\includegraphics[width=\textwidth, height=0.5\columnwidth]{figs/error-propagation.png}
\caption{\label{fig:error-propagation}
Error propagation from point (x-1,t0+t') to (x,t0+T) (1-d stencil)
}
\vspace*{-1em}
    \end{minipage}
\end{figure}

\subsection{\bf{T-step Stencil Evaluation}}

\label{sec:sec:modeling-roundoff}
%State of the art error analysis tools for round-off error bounding
%fail to work effectively and efficiently in a large problem space when using 
%SMT solvers or using search algorithms for problems with multiple nested
%loops and large iteration depths.

%
\ggcmt{The stuff below is a bit long, but avoids people reading a lot
  of math. I'll shring it later.}
%
Referring to Figure~\ref{fig:error-propagation},
the purpose of this section is to develop a methodology
whereby we can unfold the stencil $T$ steps in time,
and arrive at an ``error prediction'' for the output value at
the output $(x,t_0+T)$.
%
This will be called {\em detector precision}, $dp_T$, and
arrived at as follows:
%
\begin{compactenum}
\item Directly evaluate
the error in the range $[x-wT, x+wT]$ via all the path
coefficients leading to the output point
(these coefficients would be
as illustrated in Table~\ref{table:unroll-table}).
This relative error would be called $R_d$.

\item Also, iteratively evaluate the stencil and arrive at this output value
  by
  \begin{compactenum}
  \item (conceptually) picking all intermediate points,
    such as $P$ called
    out,
  \item finding the error flowing into $P$,
  \item find how the error
    is amplified by all the paths from $P$ to the output.
    This relative error would be called the iterated evaluation
    error that mimics the stencil evaluation itself, and termed $R_s$.
  \item suitably combining the error for all such conceptual
    points $P$ using affine arithmetic
  \end{compactenum}
\end{compactenum}
%
We can then define
\(	\hbox{bits preserved}_T  = (dp)_T = p - \log_2(\max(\boldsymbol{R_s}, \boldsymbol{R_d})) \)
which says ``remove the maximum of the uncertainties between
the direct and iterated evaluations.''
%
Our implementation uses Kahan's~\cite{kahan1996ieee} algorithm and
vectorization to ensure that $R_d$ is
minimized.
%
Thus,
the key factor impacting the number of bits preserved
will be the main stencil's iterated evaluations.
%
Soft errors or logical bugs that throw the actual error beyond
the $dp_T$ limit can then be thrown with the guarantee of
{\em no false positives}
%
\ggcmt{The stuff above is a bit long, but avoids people reading a lot
  of math. I'll shring it later.}

We extend the model of error generation and propagation to stencil codes
\footnote{Detailed modeling details are provided in the supplementary material
for the interested reader}. 
A fresh noise variable is introduced
for every floating point(FP) operation.
%
In equation$\eqref{eq:heat-unit}$, there will be 5 FP operation
for a single update generating 5 unique noise variables.
%The space complexity is linear in the number of data points involved.
The number of error variables involved is linear in the number of
data points.
%
For a d-dimensional problem with N-arrays and T-step detector model, the number of
error variables will be $O(NT^d)$.
%
The noise coefficient associated per noise variable is determined by the
specifics for that operation . 
The point $\vec{P}$ in Figure~\ref{fig:error-propagation}
shows such a point within a stencil. The total error contribution for the errors
generated at $\vec{P}$ is the accumulation of their noise coefficients scaled by
the effective path contribution(highlighted path) from $\vec{P}$
to the final output. \FPD accumulates the error for every interior point belonging
to the dependence cone of the output point to evaluate the total error.
Furthermore, doing this statically offline makes it cost efficient albeit
a conservative bound based on the input interval.
%
\ggcmt{Say it is done for exponent intervals?}
%
Thus our analysis hold for any distribution within the given input
range.

Furthermore, PDEs get more complicated with
multiple arrays corresponding to different physical quantities participating  
together. 
%Modeling EM field with finite difference time domain methods, there
%are atleast two arrays corresponding to the electric(E) and magnetic(M) fields. 
%We introduce the notion of multiple array updates.
Suppose, every update
depends on contributions from $N$ participating arrays. Let $C_{u,v,\vec{P}}$ denote the effective path
contribution from an interior point $\vec{P}$ at time $t_0+t^\prime$ in array $A_v$ towards the 
final location $x$ in array $A_u$ at time $t_0+T$. This effective path contribution can be obtained 
using automatic differentiation as in
$\eqref{eq:chain-rule}$
%
\ggcmt{Equation~\ref{eq:coeff-deriv-form} never referenced;
  also reference that here?}
%
such that
\vspace*{-0.5em}
	\begin{wrapfigure}{l}{0.4\textwidth}
    \begin{minipage}{0.4\textwidth}
\begin{equation}
\label{eq:coeff-deriv-form}
  C_{u,v,\vec{P}} = \bigg | \dfrac{dA_u[\vec{x},\!t_0\!+\!T]}{dA_v[\vec{P},t_0+t^\prime]} \bigg | 
  %\bigg | \dfrac{dA_u[\vec{x},\!t_0\!+\!T]}{dA_v[\vec{P},t_0+t^\prime]} \bigg | =
  % 											c_{(u,v,\vec{x}-\vec{P},T-t^\prime)}
\vspace*{-0.5em}
\end{equation}
	\end{minipage}
	\end{wrapfigure}

Let $E_{(\vec{P},t^\prime)}$ denotes the total error contribution at the output from freshly 
generated noise at point $\vec{P}$ in 
Figure~\ref{fig:error-propagation}. 
%it is evaluated as

%\begin{equation}
%  \label{eq:per-point-error}
%	\begin{split}
%	   E_{(\vec{P}, t^\prime)} = \sum_{\underset{\sigma^{(0)}\!\left(\!\vec{P}\! \right)}{\epsilon_i \in}}
%	   							\bigg |
%									    \overbrace{\gamma(\vec{P} , \epsilon_i)}^\text{noise coefficient}
%									\times {\rs}
%								\underbrace{C_{u,v,\vec{P}}}_\text{Propagating coefficient}
%								\bigg |
%	\end{split}
%\end{equation}

%Equation $~\eqref{eq:per-point-error}$ gives the error accumulation due to an arbitrary point $\vec{P}$ inside
%the dependence cone. 
For a stencil of neighbourhood width $\vec{w}$
%
\ggcmt{Neighborhood width? Introduce this term or
  stencil footprint width earlier when we had a
  simple 3-point stencil?}
%
around the central point, the range
of points at tile $t^\prime$ in Figure~\ref{fig:error-propagation} will extend over the integer
interval $[\vec{x} - \vec{w}(T-t^\prime), \vec{x} + \vec{w}(T-t^\prime)]$.
%
\ggcmt{What is a ``tile'' when we say Tile $t^\prime$?
Rephrase?}
%
Let $E_{u,v}^{t^\prime}$
denote the total error contribution from all points in the dependence cone from tile $t^\prime$. Then
\begin{equation}
	\label{eq:perArray-error-per-tile}
	\begin{split}
		E_{u,v}^{t^\prime} = \sum_{\underset{-\vec{w}(T-t^\prime)}{\vec{P}=}}^{\vec{w}(T-t^\prime)}
		                       E_{(\vec{P}, t^\prime)} ; \quad\hbox{where,}\quad
E_{(\vec{P}, t^\prime)} = \sum_{\underset{\sigma^{(0)}\!\left(\!\vec{P}\! \right)}{\epsilon_i \in}}
	   							\bigg |
									    \overbrace{\gamma(\vec{P} , \epsilon_i)}^\text{noise coefficient}
									\times {\rs}
								\underbrace{C_{u,v,\vec{P}}}_\text{Propagating coefficient}
								\bigg |
	\end{split}
\end{equation}

We perform this for every point inside the dependence cone. The total error$(T_E)$ 
and the relative error$(R_E)$
for point $x$ in array $A_v$ for an iteration depth of $T$ is given by

\begin{equation}
\label{eq:error-equation}
\begin{split}
	\boldsymbol{T_E}(A_u[\vec{x}, t_0+T]) &= \sum_{t^\prime=0}^{T-1}
											\bigg (
												\sum_{v=1}^N E_{u,v}^{t^\prime}
											\bigg ) ;\quad
	\boldsymbol{R_E}(A_u[\vec{x}, t_0+T]) = \bigg | \dfrac{T_E(A_u[\vec{x},t_0+T])}{A_u[\vec{x}, t_0+T]} \bigg |
\end{split}
\end{equation}

%While the total error is a quantitative measure about the volume of round-off error accumulation,
%it does not provide information about the quality of precision. For example, if the actual 
%value is close to 1, an absolute error of 0.1 would be considered large in comparison to 
%when  the actual value is in order of a million. 
The relative error measure obtained by normalizing the 
total error by the stencil value(ideally the exact real value) provides a more qualitative 
description of the precision loss.

\vspace{.5ex}
\noindent{\textbf{Iterated vs direct loss}:\/}
	Evaluating equation $~\eqref{eq:error-equation}$ for all points in the dependence cone of 
	Figure~\ref{fig:error-propagation} belonging to a bounded input interval $[I_l, I_u]$ derives the 
	relative error for the {\em iterated evaluation} of the stencil denoted by $\boldsymbol{R_s}$.
        %
        It is also possible to derive error through {\em direct evaluation} from the output
        at $t_0+T$, tracing the inputs
        all the way back to time $t_0$.
        %
	To achieve this,
        we start from $(t_0+T,\vec{x})$, and
	do a back propagation to compute the coefficient set for direct evaluation, followed by a 
	dot-product
        on the {\em entire} input data set bounded in the interval $[I_l. I_u]$.
	The back propagation of the coefficients is exactly same as the unrolling steps for 
	evaluating $\boldsymbol{R_s}$ with the key difference being that we do not propagate the
	data points but only the coeffcients. It is equivalent to assuming that the data points are all one.
	This gives the effect of accumulating the effective coefficents without any interference
	from the data points. At the end, a large dot product is computed over the effective coefficients
	with the data points forming the support for the Tstep where we now include back the interval.
	To minimize round-off error in the large dot-product we use kahan's summation which has a
	bound for large summation resulting in just extra 2 ulp loss(ignoring second order effects).

	% Kahan mentioned later
	%To compensate
	%for high round-of error accumulation due to large dot-product, we deploy kahan's algorithm
	%~\cite{kahan1996ieee}, which is computationally more expensive but more
	%precision-preserving summation algorithm. To compensate for the increased compute cost
	%we further vectorize it manually .

        
        The main factor driving the round-off error in direct evaluation is {\em coefficient extraction}
        (as illustrated in Table~\ref{table:unroll-table}).
        %
        This can be performed
        offline at a high precision (much higher than
	working precision) to further minimize the precision loss.
        %
        Let the relative error term 
	evaluated for the direct evaluation be $\boldsymbol{R_d}$.
        The conservatively estimated number of bits 
	preserved at the detector output can then be expressed as
   \(	\hbox{bits preserved}_T  = (dp)_T = p - \log_2(\max(\boldsymbol{R_s}, \boldsymbol{R_d})) \).
   %}
   %
{\tiny This   
equation
evaluates the upper bound on the minimum matching precision between the
iterated and direct evaluation schemes over T-steps that survives the loss due to 
roundoff error.}
\ggcmt{The above key sentence comes muddled. Rewrote it below.}
This equation finds the maximum uncertainty due to roundoff, and
removes it from $p$.
%
This is denoted by \textbf{detector precision($dp_T$)},
and represents the {\em maximum precision}
 that can potentially be guaranteed by our detection
 strategy.

Our optimizations use Kahan's~\cite{kahan1996ieee} algorithm and vectorize
the evaluation to ensures that $R_d$ is
minimized.
%
This ensures that the key factor impacting the number of bits preserved
is the main stencil's iterated evaluations.
Note that our error analysis is conservative in its treatment of
input values,
and might not capture the maximum precision preserved by a specific
set of input values.
On the other hand,
it provides a rigorous detection guarantee and attempts to
minimize total cost in providing that guarantee.




